A Contrastive Learning Approach for Training Variational Autoencoder Priors

Variational autoencoders (VAEs) are one of the powerful likelihood-based generative models with applications in many domains. However, they struggle to generate high-quality images, especially when samples are obtained from the prior without any tempering. One explanation for VAEs' poor generative quality is the prior hole problem: the prior distribution fails to match the aggregate approximate posterior. Due to this mismatch, there exist areas in the latent space with high density under the prior that do not correspond to any encoded image. Samples from those areas are decoded to corrupted images. To tackle this issue, we propose an energy-based prior defined by the product of a base prior distribution and a reweighting factor, designed to bring the base closer to the aggregate posterior. We train the reweighting factor by noise contrastive estimation, and we generalize it to hierarchical VAEs with many latent variable groups. Our experiments confirm that the proposed noise contrastive priors improve the generative performance of state-of-the-art VAEs by a large margin on the MNIST, CIFAR-10, CelebA 64, and CelebA HQ 256 datasets. Our method is simple and can be applied to a wide variety of VAEs to improve the expressivity of their prior distribution.

==> figs/gaussian_synthetic_data_fig.tex <==
\begin{figure*}[t!]
	\centering
	 \setlength\tabcolsep{0pt}
% 	 \vspace{-0.15cm}
	\begin{tabular}{ccc}
        \includegraphics[width=0.3\linewidth]{figs/rebuttal/grid_true_data_samples.jpg} \hspace{0.01cm} &
        \includegraphics[width=0.3\linewidth]{figs/rebuttal/grid_vae_pz_samples.pdf}
        \hspace{0.01cm}&
        \includegraphics[width=0.3\linewidth]{figs/rebuttal/grid_ncp_reweighted_samples.pdf} \\
        % \vspace{-0.1cm}
	    {(a) Samples from the true distribution}&	{(b) Samples from VAE} & {(c) Samples from NCP-VAE}
	    \end{tabular}
	\caption{Qualitative results on mixture of 25-Gaussians. Fig.(a) shows the true distribution samples. Note that the samples decoded from the base prior $p(\bz)$ without the NCP approach generates many points in the the low density regions under the data distribution, (Fig. (b)). These points are removed using our NCP approach (Fig. (c)).}
	\label{fig:gaussian grid}
% 	\vspace{-1cm}
\end{figure*}

==> rebuttal/minst_table.tex <==
\begin{table}[t]
\vspace{-0.1cm}
\small
\begin{minipage}{\columnwidth}
    \centering
\caption{Likelihood results on MNIST on single latent group model with architecture from SNIS~\citep{lawson2019energy} (in nats).}
\label{tab:mnist latent sclaing}
   \begin{tabular}{lll}
      Latent Dim & \makecell{NLL \\ (lower bound)} & \makecell{NLL \\ (upper bound)} \\
      \midrule
      50 & 82.82 & 82.42\\ 
      100  & 83.17 & 83.05\\
      1000  & 83.54 & 83.48\\
\bottomrule
\end{tabular}
\end{minipage}
\vspace{-0.5cm}
\end{table}

==> rebuttal/snis_time_memory.tex <==
\begin{table}[t]
\vspace{-0.2cm}
\small
\begin{minipage}{\columnwidth}
    \centering
\caption{Time \& Memory comparison with  SNIS~\citep{lawson2019energy} for 128 proposals. Time-$N$ is the time used to generate a batch of $N$ images.}
\label{tab:snis time and memory}
   \begin{tabular}{lllll}
      Method &\makecell{Time -1 \\ (sec)} & \makecell{Time-10 \\ (sec)} & \makecell{Time-5000 \\ (sec)} & \makecell{Memory\\ (MB)} \\
      \midrule
      SNIS~\citep{lawson2019energy} & 0.004 & 0.004 & 0.025 & 275\\ 
      NCP  & 0.001 & 0.002 & 0.027 & 543\\
  
\bottomrule
\end{tabular}
\end{minipage}
\vspace{-0.6cm}
\end{table}


==> sections/80-checklist.tex <==
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{see Section~\ref{sec:related}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{see Section~\ref{sec:impact}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{see Section~\ref{sec:background} and \ref{sec:method}}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{see Appendix~\ref{app:variational lower bound} and \ref{app:cnce}}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The base code for~\citep{vahdat2020NVAE} is public, see Appendix~\ref{app:classifier_architecture} for implementing our NCP approach.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{see Appendix~\ref{app:classifier_architecture}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{The numbers in all tables are averaged over 5 runs}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{~\tabref{tab:sirAblation} provides time and memory usage. We use 15 NVIDIA Tesla V100, 32GB GPUs to train the binary classifiers in parallel.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{see Section~\ref{subsec:quan_res_ncpvae}}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> sections/rebuttal.tex <==
\section{Rebuttal}
We demonstrate the efficacy of our approach on a synthetic dataset. In Fig.~\ref{fig:gaussian grid} we use the 25-Gaussians dataset, that is generated by a mixture of 25 two-dimensional Gaussian distributions that are arranged on a grid. The encoder and decoder of the VAE have 4 fully connected layers with 256 hidden units, with 20 dimensional latent variables. The discriminator has 4 fully connected layers with 256 hidden units.

Note that the samples decoded from the prior p(z) Fig.~\ref{fig:gaussian grid}(b)) of the VAE without the noise contrastive approach generates many points from the 'holes' of the original data. These are removed by using the our NCP approach (Fig.~\ref{fig:gaussian grid}(c)).
\begin{figure*}[h!]
	\centering
	 \setlength\tabcolsep{0pt}
	\begin{tabular}{ccc}
        \includegraphics[width=0.32\linewidth]{figs/rebuttal/grid_true_data_samples.jpg} \hspace{0.01cm} \vspace{0.1cm}&
        \includegraphics[width=0.32\linewidth]{figs/rebuttal/grid_vae_pz_samples.pdf}
        \hspace{0.01cm}\vspace{0.1cm}&
        \includegraphics[width=0.32\linewidth]{figs/rebuttal/grid_ncp_reweighted_samples.pdf} \\
        \vspace{0.1cm}
	    {(a) Samples from the true distribution}&	{(b) Samples from VAE} & {(c) Samples from NCP-VAE}
	    \end{tabular}
	\caption{Qualitative results on mixture of 25-Gaussians.}
	\label{fig:gaussian grid}
	\vspace{-0.1cm}
\end{figure*}

\subsection{Additional Comparisons to Prior Art}

{\bf{Single Group Latent Space}}: In Tab.~\ref{tab:single latent celeba 64} we show the generative performance of our approach applied to the VAE architecture in RAE~\citep{ghosh2020deterministicVAE}. Note that the same VAE architecture used in 2s-VAE~\citep{dai2018diagnosing} and WAE~\citep{tolstikhin2018wassersteinAE}. The experiments are performed on CelebA-64 dataset. Our NCP-VAE improves the performance on the base VAE, improving the FID to 41.44 from 48.12. Additionally, when NCP is applied to the samples from GMM (proposed in RAE), it improves the performance of RAE to FID of 39.00. Note for this section we re-implemented the VAE model in ~\citep{ghosh2020deterministicVAE}. 

In Tab.~\ref{tab:table mnist single latent} we evaluate the negative log-likelihood (NLL) for MNIST. We follow the approach of \citep{lawson2019energy} to obtain the lower bound on the log likelihood. NCP-VAE obtainnd NLL of 82.82 which is comparable to~\citep{lawson2019energy} (82.52), while outperforming LARS ~\citep{bauer2019resampledPrior} and NLL using samples from a Gaussian prior(84.82). We trained our own model following the architecture in~\citep{lawson2019energy}.
\input{tables/rebuttal_table}

\newpage
\section{Additional Qualitative Examples} \label{app:qual celeb 64 rebuttal}
In Fig.~\ref{fig:comparison nvae ncp-vae qual celeb 64} we show additional examples of images generated by NVAE~\citep{vahdat2020NVAE} and our NCP-VAE. We use temperature 0.7 for both the methods.
\begin{figure*}[h!]
    \centering
    \includegraphics[scale=0.5]{figs/rebuttal/nvae_cherries_celeba_64_t=0.7.png}\\ Random Samples from NVAE at $t = 0.7$\\
    
    \includegraphics[scale=0.5]{figs/rebuttal/ncpvae_cherries_celeba_64_t=0.7.png}
    \\ Random Samples from NCP-VAE at $t = 0.7$\\
    \caption{ Additional samples from CelebA-64 at $t = 0.7$. }
    \label{fig:comparison nvae ncp-vae qual celeb 64}
\end{figure*}

==> tables/RAE_results.tex <==
%\vspace{-0.25cm}
\begin{table}[h!]
\small
\begin{minipage}{\columnwidth}
    \centering
\caption{Comparison with two-stage VAEs on CelebA-64 with RAE~(\citeauthor{ghosh2020deterministicVAE}) networks. \textsuperscript{$\dagger$} Results reported by~\citeauthor{ghosh2020deterministicVAE}.}
\label{tab:single latent celeba 64}
   \begin{tabular}{ll}
    Model & FID$\downarrow$\\
    \midrule
    VAE w/ Gaussian prior  & 48.12\textsuperscript{$\dagger$} \\
    2s-VAE~\citep{dai2018diagnosing} & 49.70\textsuperscript{$\dagger$}\\
    WAE~\citep{tolstikhin2018wassersteinAE} & 42.73\textsuperscript{$\dagger$}\\
    RAE~\citep{ghosh2020deterministicVAE} & 40.95\textsuperscript{$\dagger$}\\
    \hline
    NCP w/ Gaussian prior as base & 41.28 \\
    NCP w/ GMM prior as base & \bf{39.00}\\
    \hline
    Base VAE-{\color{blue}Recon} & 36.01\\
\bottomrule
\end{tabular}
\end{minipage}
\vspace{-0.3cm}
\end{table}


==> tables/SNIS_results.tex <==
\begin{table}[h!]
\small
\begin{minipage}{\columnwidth}
    \centering
\caption{Likelihood results on MNIST on single latent group model with architecture
from LARS~\citep{bauer2019resampledPrior} \& SNIS~\citep{lawson2019energy} (results in nats). We closely follow the training hyperparameters used by \citet{lawson2019energy}}
\label{tab:table mnist single latent}
   \begin{tabular}{ll}
      Model & NLL$\downarrow$ \\
      \midrule
      VAE w/ Gaussian prior & 84.82 \\
      VAE w/ LARS prior~\citep{bauer2019resampledPrior} & 83.03 \\
      VAE w/ SNIS prior~\citep{lawson2019energy}   & \bf 82.52\\
      \hline
    NCP-VAE & 82.82\\
\bottomrule
\end{tabular}
\end{minipage}
\vspace{-0.35cm}
\end{table}

==> tables/celebA_64.tex <==
\vspace{-0.3cm}
\begin{table}[th]
\small
\begin{minipage}{\columnwidth}
    \centering
\caption{Generative performance on CelebA-64}
\label{tab:table celeba 64}
   \begin{tabular}{ll}
      Model & FID$\downarrow$ \\
      \midrule
      NCP-VAE (ours) & \bf 5.25\\
      VAEBM \citep{xiao2021vaebm} & 5.31 \\
      NVAE \citep{vahdat2020NVAE} & 13.48\\
      \hline
      RAE \citep{ghosh2020deterministicVAE} & 40.95  \\
      2s-VAE \citep{dai2018diagnosing}& 44.4 \\
      WAE \citep{tolstikhin2018wassersteinAE} & 35 \\
      Perceptial AE\citep{zhang2019perceptual} & 13.8 \\
      \hline
      Latent EBM \citep{pang2020EBMPrior} & 37.87 \\
    %   Flow CE \citep{gao2020flow} & 12.21\\
    %   Divergence Triangle \citep{han2020joint} & 24.7 \\
      \hline
      \hline
      %NCSNv2 \citep{song2020improved} & 26.86 \\
      %\hline
      COCO-GAN \citep{lin2019coco} & 4.0 \\
      QA-GAN \citep{parimala2019quality} & 6.42 \\
      \hline
      NVAE-{\color{blue}Recon} \citep{vahdat2020NVAE} & 1.03\\
\bottomrule
 \end{tabular}
\end{minipage}\hfill
\end{table}

==> tables/celeba_256.tex <==
\begin{table}[th]
\vspace{0.1cm}
\small
\begin{minipage}{\columnwidth}
    \centering
\caption{Generative results on CelebA-HQ-256}
\label{tab:table celeba 256}
  \begin{tabular}{ll}
      Model & FID$\downarrow$ \\
      \midrule
      NCP-VAE (ours) & 24.79\\
      VAEBM \citep{xiao2021vaebm} &  \bf 20.38 \\
      NVAE \citep{vahdat2020NVAE} & 40.26\\
      \hline
      GLOW \citep{kingma2018glow} & 68.93\\
      \hline
      \hline
      Advers. LAE \citep{pidhorskyi2020adversarial} & 19.21\\
      PGGAN \citep{karras2017progressive} & 8.03 \\
      \hline
      NVAE-{\color{blue}Recon} \citep{vahdat2020NVAE} & 0.45\\
\bottomrule
\end{tabular}
\end{minipage}\hfill
\vspace{-0.1cm}
\end{table}

==> tables/cifar10.tex <==
\vspace{-0.3cm}
\begin{table}[th]
\small
\begin{minipage}{\columnwidth}
    \centering
\caption{Generative performance on CIFAR-10}
\label{tab:table cifar 10}
  \begin{tabular}{ll}
      Model & FID$\downarrow$\\
      \midrule
      NCP-VAE (ours) &  24.08 \\
      VAEBM \citep{xiao2021vaebm} & \bf 12.96 \\
      NVAE \citep{vahdat2020NVAE} & 51.71 \\
      \hline
      RAE \citep{ghosh2020deterministicVAE} & 74.16  \\
      2s-VAE \citep{dai2018diagnosing}& 72.9 \\
      Perceptial AE \citep{zhang2019perceptual} & 51.51 \\
      \hline
      EBM \citep{du2019implicit} & 40.58 \\
      Latent EBM \citep{pang2020EBMPrior} & 70.15 \\
      \hline
      \hline
      Style-GANv2 \citep{karras2020training} & 3.26 \\
      Denoising Diffusion Process \citep{ho2020denoising} & 3.17 \\ 
    %   Flow CE \citep{gao2020flow} & 12.21\\
    %   Divergence Triangle \citep{han2020joint} & 24.7 \\
    %   \hline
    %   \hline
    %   %NCSNv2 (\citep{song2020improved}) & 26.86 \\
    %   %\hline
    %   COCO-GAN \citep{lin2019coco} & 4.0 \\
    %   QA-GAN \citep{parimala2019quality} & 6.42 \\
\hline
NVAE-{\color{blue}Recon} \citep{vahdat2020NVAE} & 2.67\\
\bottomrule
 \end{tabular}
\end{minipage}\hfill
\vspace{-0.6cm}
\end{table}

==> tables/mnist.tex <==
\begin{table}[th]
\vspace{-0.3cm}
\small
\begin{minipage}{\columnwidth}
    \centering
\caption{Likelihood results on MNIST in nats}
\label{tab:table mnist}
  \begin{tabular}{ll}
      Model & NLL$\downarrow$ \\
      \midrule
      NCP-VAE (ours) & \bf 78.10\\
      NVAE-small \citep{vahdat2020NVAE}    & 78.67\\
      \hline
      % NVAE-original \citep{vahdat2020NVAE} & 78.01\\
      BIVA \citep{maaloe2019biva} & 78.41 \\
      DAVE++ \citep{Vahdat2018DVAE++} & 78.49 \\
      IAF-VAE \citep{kingma2016improved} & 79.10 \\
      VampPrior AR dec. (\citeauthor{tomczak2018VampPrior}) & 78.45 \\
    %   \hline
    %   \hline
    %   Advers. LAE \citep{pidhorskyi2020adversarial} & 19.21\\
    %   PGGAN \citep{karras2017progressive} & 8.03 \\
\bottomrule
\end{tabular}
\end{minipage}
\vspace{-0.3cm}
\end{table}

